Repelling Random Walks

We present a novel quasi-Monte Carlo mechanism to improve graph-based sampling, coined repelling random walks. By inducing correlations between the trajectories of an interacting ensemble such that their marginal transition probabilities are unmodified, we are able to explore the graph more efficiently, improving the concentration of statistical estimators whilst leaving them unbiased. The mechanism has a trivial drop-in implementation. We showcase the effectiveness of repelling random walks in a range of settings including estimation of graph kernels, the PageRank vector and graphlet concentrations. We provide detailed experimental evaluation and robust theoretical guarantees. To our knowledge, repelling random walks constitute the first rigorously studied quasi-Monte Carlo scheme correlating the directions of walkers on a graph, inviting new research in this exciting nascent domain.

==> eli_proof.tex <==
\subsection{proof that repelling reduces variance}

\begin{definition}
Let $w = (v_0, \ldots, v_k)$ be a walk in some graph, and let $t \in \{0, \ldots, k\}$. Then we write 

$$w\upharpoonright_t = (v_0, \ldots, v_t)$$

$$w\upharpoonright^t = (v_t, \ldots, v_k)$$
\end{definition}


Let $G=(V,E)$ be a finite graph and, let $r \in V$, let $m \in \mathbb{N}$, let $p_{term} \in (0,1)$ and let $S \subseteq (\mathbb{N} \cup \{0\}) \times V \times 2^{\{1, \ldots, m\}}$. We define the $S$-repelling random algorithm for generating $m$ walks as follows:

\begin{enumerate}

\item FOR all $\alpha \in \{1, \ldots, m\}$

\item \quad Set $w_\alpha = (r)$ (the one-vertex walk with only $r$ in it).

\item \quad With probability $p_{term}$ declare $w_\alpha$ as terminated.

\item Set $t=0$.

\item WHILE unterminated paths exist

\item \quad FOR all $v \in V$

\item \quad \quad Set $k = d(v)$.

\item \quad \quad Set $X$ as the set of all $\alpha$ such that $w_\alpha$ is unterminated and currently ends at $v$.

\item \quad \quad IF $(t,v,X) \in S$

\item \quad \quad \quad Set $Y=X$.

\item \quad \quad \quad WHILE $Y \neq \emptyset$

\item \quad \quad \quad \quad IF $|Y| \leq k$

\item \quad \quad \quad \quad \quad Set $Z = Y$.

\item \quad \quad \quad \quad ELSE

\item \quad \quad \quad \quad \quad Set $Z$ as the set of $k$ minimal indices in $Y$.

\item \quad \quad \quad \quad Choose a one-to-one function $f: Z \to N(v)$ uniformly at random.

\item \quad \quad \quad \quad FOR all $\alpha \in Z$

\item \quad \quad \quad \quad \quad Add $f(\alpha)$ at the end of $w_\alpha$.

\item \quad \quad \quad \quad \quad With probability $p_{term}$ declare $w_\alpha$ as terminated.

\item \quad \quad \quad \quad Set $Y = Y \setminus Z$.

\item \quad \quad ELSE

\item \quad \quad \quad FOR all $\alpha \in X$

\item \quad \quad \quad \quad Choose a neighbour $u$ of $v$ uniformly at random.

\item \quad \quad \quad \quad Add $u$ at the end of $w_\alpha$.

\item \quad \quad \quad \quad With probability $p_{term}$ declare $w_\alpha$ as terminated.

\item \quad Set $t = t+1$.

\end{enumerate}

We observe that for a walk $w$ starting on $r$, the probability $p(w_\alpha = w)$ depends on neither $\alpha$ nor $S$. Also, note that for two walks $w, w'$ both starting on $r$ satisfying $w\upharpoonright^t= w'\upharpoonright^t$, for some $t$, we have $p(w_\alpha = w | w_\alpha\upharpoonright_t = w\upharpoonright_t) = p(w_\alpha = w' | w_\alpha\upharpoonright_t = w'\upharpoonright_t)$. This makes the following notations well-defined:

$$p_0(w) = p(w_\alpha = w)$$

$$p_t(w\upharpoonright^t) = p(w_\alpha = w | w_\alpha\upharpoonright_t = w\upharpoonright_t)$$

Note that for $S = \emptyset$ we get the i.i.d. model and for $S = (\mathbb{N} \cup \{0\}) \times V \times 2^{\{1, \ldots, m\}}$, we get the repelling model. 

Let $W_r$ denote the set of all finite walks starting from $r$. A function $y: W_r \to \mathbb{R}$ is called {\em step-by-step linear} if it can be written as

$$y(v_0, \ldots, v_k) = 
\sum_{i=1}^k f(v_i,i) \prod_{j=1}^i g(\{v_{j-1},v_j\},j)$$

for some $f: V \times \mathbb{N} \to \mathbb{R}$ and $g: E \times \mathbb{N} \to \mathbb{R}^+$.

Note that for $w = (v_0, \ldots, v_k) \in W_r$ and $t \in \{0, \ldots, k\}$ we can write

$$y(w) = a(w\upharpoonright_t)x(w\upharpoonright^t)+y(w\upharpoonright_t)$$

where $a(v_0, \ldots, v_t) = \prod_{j=1}^t g(\{v_{j-1},v_j\},j)$ and $x(v_t, \ldots, v_k) = \sum_{i=t+1}^k f(v_i,i) \prod_{j=t+1}^i g(\{v_{j-1},v_j\},j)$.


The superiority of the repelling model is a special case of the following theorem (when taking $S_1 = \emptyset$ and $S_2 = (\mathbb{N} \cup \{0\}) \times V \times 2^{\{1, \ldots, m\}}$).

\begin{theorem}
Let $S_1 \subseteq S_2 \subseteq (\mathbb{N} \cup \{0\}) \times V \times 2^{\{1, \ldots, m\}}$. 
Let $y : W_r \to \mathbb{R}$ be a step-by-step linear function and 
For each $i \in \{1,2\}$, let $Y_i$ be the 
random variable 
$y(w_1)+ \ldots + y(w_m)$, where $w_1, \ldots, w_m$ are the walks generated in the above random algorithm when taking $S = S_i$. If $VAR(Y_1)$ and $VAR(Y_2)$ are finite and for each $(t_1, v_1, X_1) \in S_1$ and $(t_2, v_2, X_2) \in S_2 \setminus S_1$ we have $t_1 \leq t_2$, then

$$VAR(Y_1) \leq VAR(Y_2)$$
\end{theorem}

\begin{proof}
It is enough to prove the theorem in the case that $S_2 \setminus S_1$ is a singleton, say, 
$S_2 \setminus S_1 = \{(t_0,v_0,X_0)\}$. Then by induction we can prove the theorem in all the case where 


Let $E_1$ denote the expectancy when taking $S=S_1$ and let $E_2$ denote the expectancy when taking $S=S_2$. Let $w'_1, \ldots, w'_m$ be walks of length $t_0$ starting from $r$ and let $A$ denote the event that $w_i \upharpoonright_{t_0} = w'_i$ for all $i \in \{1, \ldots, m\}$. 

Consider the state in the algorithm when $t=t_0$ and $v=v_0$. Then $k=d(v)$. Denote the neighbours of $v$ by $u_1, \ldots, u_k$. For each $i \in \{1, \ldots, k\}$ we enumerate the finite walks starting at $u_i$ as $(w''_{ij})_{j \in \mathbb{N}}$. We write $p_{ij} = p_{t+1}(w''_{ij})$, so clearly $\sum_{j=1}^\infty p_{ij} = 1$. We write $w'''_{ij}$ for the walk obtained from $w''_{ij}$ by adding $v$ as the first vertex. 

Take two of the walks obtained by the algorithm, say $w_\alpha$ and $w_\beta$. We claim that $E_1(y(w_\alpha)y(w_\beta)|A) \geq E_2(y(w_\alpha)y(w_\beta)|A)$. If the value of $X$ calculated in this state of the algorithm is not $X_0$, then clearly $E_1(y(w_\alpha)y(w_\beta)|A) = E_2(y(w_\alpha)y(w_\beta)|A)$, so we may assume $X=X_0$. Similarly, we may assume that at some point we have $\{alpha, \beta\} \in Z$.

As discussed above, there are functions a,x,b, such that for every $w \in W_r$ we have

$$y(w) = a(w\upharpoonright_t)x(w\upharpoonright^t)+y(w\upharpoonright_t)$$

Write $a_\alpha = a(w'_\alpha), a_\beta = a(w'_\beta), b_\alpha = b(w'_\alpha), b_\beta = b(w'_\beta)$ and $x_{ij} = x(w'''_{ij})$.

We can now calculate:

$$E_1(y(w_\alpha)y(w_\beta)|A) = 
\sum_{i=1}^k\sum_{j=1}^\infty
\sum_{i'=1}^k\sum_{j'=1}^\infty
\frac{p_{i,j}p_{i'j'}}{k^2}
(a_\alpha x_{ij} + b_\alpha) 
(a_\beta x_{i'j'} + b_\beta)$$

$$E_2(y(w_\alpha)y(w_\beta)|A) = 
\sum_{i=1}^k\sum_{j=1}^\infty \,
\sum_{i' \in \{1, \ldots, k\} \setminus \{i\}} 
\,
\sum_{j'=1}^\infty
\frac{p_{i,j}p_{i'j'}}{k(k-1)}
(a_\alpha x_{ij} + b_\alpha) 
(a_\beta x_{i'j'} + b_\beta)$$

When subtracting, all terms with $b_\alpha$ and/or $b_\beta$ cancel, and we get

$$E_1(y(w_\alpha)y(w_\beta)|A)
- E_2(y(w_\alpha)y(w_\beta)|A) = $$

$$
\sum_{i=1}^k\sum_{j=1}^\infty
\sum_{j'=1}^\infty
\frac{p_{i,j}p_{ij'}}{k^2}
a_\alpha x_{ij} 
a_\beta x_{ij'}-
\sum_{i=1}^k\sum_{j=1}^\infty \,
\sum_{i' \in \{1, \ldots, k\} \setminus \{i\}} 
\,
\sum_{j'=1}^\infty
\frac{p_{i,j}p_{i'j'}}{k^2(k-1)}
a_\alpha x_{ij} 
a_\beta x_{i'j'}$$

$$ = \frac{a_\alpha a_\beta}{k^2(k-1)}
\sum_{i=1}^{k-1}\sum_{i'=i+1}^k
\left(
\sum_{j=1}^\infty p_{ij} x_{ij} - 
\sum_{j'=1}^\infty p_{i'j'} x_{i'j'}
\right)^2 \geq 0
$$

Since this is true for any event $A$ corresponding to any $w'_1, \ldots, w'_m$, we have $E_1(y(w_\alpha)y(w_\beta)) \geq
E_2(y(w_\alpha)y(w_\beta))$. Also, note that 
$E_1(y(w_\alpha)^2) =
E_2(y(w_\alpha)^2$, since the choice of $S$ does not affect the distribution of $w_\alpha$. Hence

$$
E(Y_1^2) = E_1((\sum_{\alpha=1}^m y(w_\alpha))^2) \geq 
E_2((\sum_{\alpha=1}^m y(w_\alpha))^2) = E(Y_2^2)
$$

On the other hand, clearly $E(Y_1) = E(Y_2)$, and therefore $VAR(Y_1) \geq VAR(Y_2)$.
\end{proof}

==> iclr2024/deprecated.tex <==
\subsection{Uncertainty propagation on the graph}
    With both sampling strategies $1$ and $2$, each timestep can be divided into a $p$-step (where every walker terminates with probability $p$) and a $d$-step (where every surviving walker moves to a neighbour according to the particular sampling strategy). We will begin by considering the effect of the $d$-step on the distribution over $N_i$.  

Concretely, suppose that we have $N_i'$ walkers at a particular node (\emph{after} the $p$-step), where $N_i'$ is a random variable with finite mean and variance. What will be the variance of the random variable $N_{i+1}$, the number of walkers at a neighbouring node? 

With the i.i.d. sampling strategy, it is straightforward to convince oneself that
\begin{equation} \label{eq:prop_iid}
    \textrm{Var}(N_{i+1}) = \frac{\textrm{Var}(N_i')}{d^2} + \frac{\mathbb{E}(N_i')}{d}\left(1-\frac{1}{d} \right), 
\end{equation}
which follows from the properties of the Binomial distribution. Strategy $2$ is more subtle; the $d$-step takes $N_i' \to N_i' // d + \eps$, where $\eps$ is a random variable equal to $1$ with probability $\frac{N_i' \% d}{d}$ and $0$ otherwise. Working through the algebra,
\begin{equation} \label{eq:prop_new}
    \textrm{Var}(N_{i+1}) = \frac{\textrm{Var}(N_i')}{d^2} + \mathbb{E} \left[\frac{N_i' \% d}{d} \left( 1 - \frac{N_i' \% d}{d} \right) \right]. 
\end{equation}
It is trivial see that the second term in Eq. \ref{eq:prop_new} is upper bounded by the second term in Eq. \ref{eq:prop_iid}. It follows that the variance on $N_i$ induced by strategy $2$ is upper bounded by the variance on strategy $1$. 

Note also that the variance on number of walkers \emph{after} the $p$-step is simply related to the variance on the number \emph{before}: $\textrm{Var}(N_i') = \textrm{Var}(N_i)(1-p)^2 + \mathbb{E}(N_i)p(1-p)$. The difference in variance between strategies $1$ and $2$ is:
\begin{equation}
    \Delta \textrm{Var}(N_{i+1})  = \Delta \textrm{Var}(N_{i}) \left(\frac{1-p}{d} \right)^2 + f(N_i)
\end{equation}
where $f(N_i)$ is a \emph{functional} over the space of probability distributions $p(N_i)$, defined by
\begin{equation}
    f(N_i) \coloneqq \mathbb{E} \left[ \frac{N_i'}{d} \left(1-\frac{1}{d} \right) -  \frac{N_i' \% d}{d} \left( 1 - \frac{N_i' \% d}{d} \right)\right] \geq 0.
\end{equation}
Here, the variable $N_i'$ is obtained from $N_i$ via the $p$-step. Taking $N_0 \sim \delta(N_0 - N)$ such that $\textrm{Var}(N_0) = 0$, we conclude that
\begin{equation}
    \Delta \textrm{Var}(N_{i+1}) = \sum_{j=0}^i f(N_{j}) \left(\frac{1-p}{d} \right)^{2(i-j)} \geq 0. 
\end{equation}

This is intuitive. Distributing walkers more evenly between neighbours suppresses the variance on $N_i$.

\begin{figure}
    \centering
    \includegraphics[width = 0.4\linewidth]{iclr2023/images/IMG_0993.png}
    \caption{Schematic of walks $\omega_{ix}$ and $\omega_{iy}$ that diverge at node $0$.}
    \label{fig:walks_schematic}
\end{figure}

Let us now consider the behaviour of $N(\omega_{ix}) N(\omega_{iy})$ -- namely, \textbf{off-diagonal} terms of $(\phi(i)^\top \phi(j))^2$. Suppose that the walks begin together at node $i$ and wlg share the same path to node $0$, after which they diverge to nodes $x$ via $1$ and $y$ via $2$ respectively. Then we have that
 \begin{equation}
     \mathbb{E}(N_x N_y ) = \int \mathbb{E}(N_x | N_1) \mathbb{E}(N_y | N_2) p(N_1 N_2 | N_0) p(N_0 | N_i) p(N_i) \mathrm{d}N_i \mathrm{d}N_0 \mathrm{d}N_1 \mathrm{d}N_2. 
 \end{equation}
 It is straightforward to see that $\mathbb{E}(N_x | N_1) = N_1 \left( \frac{1-p}{d}\right)^{\textrm{len}(\omega_{0x})-1}$ and $\mathbb{E}(N_y | N_2) = N_2 \left( \frac{1-p}{d}\right)^{\textrm{len}(\omega_{0y})-1}$, whereupon
 \begin{equation}
\mathbb{E}(N_x N_y) = \mathbb{E}(N_1 N_2) \left( \frac{1-p}{d}\right)^{\textrm{len}(\omega_{0x}) + \textrm{len}(\omega_{0y})-2}.
\end{equation}
What is $\mathbb{E}(N_1 N_2)$? First, consider a fixed value for $N_0'$ (number of walkers at node $0$ after the $p$-step), $\mathbb{E}(N_1 N_2 | N_0')$. Then
\begin{equation}
N_1 \sim N_0' // d + \epsilon_1
\end{equation}
\begin{equation}
N_2 \sim N_0' // d + \epsilon_2
\end{equation}
where $\epsilon_1$ and $\epsilon_2$ are anticorrelated random variables that can take values $0$ or $1$. Denoting the remainder  $R \coloneqq N_0' \% d$, it is straightforward to arrive at the following: 
\begin{table}[H]
    \centering  
    \begin{tabular}{c c | c}
    \toprule
        $\epsilon_1$ & $\epsilon_2$ & $p(\epsilon_1, \epsilon_2)$ \\ \midrule
         0 & 0 & $\frac{(d-R)(d-R-1)}{d(d-1)}$\\
         1 & 0 & $\frac{R(d-R)}{d(d-1)}$\\
         0 & 1 & $\frac{R(d-R)}{d(d-1)}$ \\
         1 & 1 & $\frac{R(R-1)}{d(d-1)}$\\
         \bottomrule
    \end{tabular}
    \label{tab:my_label}
\end{table}
It follows immediately that
\begin{equation}
    \mathbb{E}(\eps_1 \eps_2 ) = \frac{R(R-1)}{d(d-1)},
\end{equation}
\begin{equation}
\mathbb{E}(\epsilon_1) = \mathbb{E}(\epsilon_2) = \frac{R}{d}.  
\end{equation}
Therefore, 
\begin{equation} \label{eq:vector_off_diag}
\begin{multlined}
\mathbb{E}(N_1 N_2 | N_0' ) = \left(\frac{N_0 ' }{d} \right)^2 + \mathbb{E}(\epsilon_1 \epsilon_2) - \mathbb{E}(\epsilon_1)\mathbb{E}(\epsilon_2)     
\\ = \left(\frac{N_0 ' }{d} \right)^2 + \frac{R}{d} \left( \frac{R-1}{d-1} - \frac{R}{d} \right)
\end{multlined}
\end{equation}
which shows that $N_1$ and $N_2$ are anticorrelated. With strategy $1$, the analogous form is
\begin{equation} \label{eq:iid_off_diag}
\begin{multlined}
\mathbb{E}(N_1 N_2 | N_0') = \sum_{l_1 = 1}^{N_0'} \sum_{l_2 = 1}^{N_0'} \mathbb{I}(\omega_{01} \in \bar{\Omega}_{l_1} ) \mathbb{I}(\omega_{02} \in \bar{\Omega}_{l_2})   
\\ = \left( \frac{N_0'}{d} \right)^2 - \frac{N_0 '}{d^2}. 
\end{multlined}
\end{equation}
Carefully comparing Eqs \ref{eq:vector_off_diag} and \ref{eq:iid_off_diag}, we have that
\begin{equation} \label{eq:cross_terms}
    \Delta \mathbb{E}(N_x N_y) = \left( \frac{\Delta \textrm{Var}(N_0)}{d^2} - \frac{f(N_0)}{d-1} \right) \left( \frac{1-p}{d}\right)^{\textrm{len}(\omega_{0x}) + \textrm{len}(\omega_{0y})-2}  
\end{equation}
where $0$ denotes the node at which the walks diverge (not to be confused with the number of walkers at the first node).

Now we have a problem. The first term in Eq. \ref{eq:cross_terms} is positive but the second term is negative. Intuitively, out scheme helps suppress the variance on the number of particles \emph{at} the point of divergence $0$, but given any such number the negative correlations between the number arriving at $x$ and $y$ are weaker (almost by construction). When the second term dominates -- e.g. when the walks diverge early -- $\mathbb{E}(N_x N_y)$ will \emph{not} be reduced. So not every term in $\mathbb{E}(\phi(i)^\top \phi(j) )$ is suppressed and we have to work harder. 

\subsubsection{Special case: $N_0 < d$}
Now consider the special case that the initial number of particles is smaller than the node degree, $N_0 < d$. It follows that $N_i < d \hspace{2mm} \forall \hspace{2mm} i$, whereupon $N_i' \% d = N_i'$. This enables us to obtain explicit closed-form expressions for the variance on $N_i$. After just a little work,

\begin{equation}
    \textrm{Var}(N_i) = \begin{cases}
        0 & \textrm{if $i=0$}, \\ 
        \begin{cases}
        N_0 \left( \frac{1-p}{d} \right)^i \left( 1 - \left( \frac{1-p}{d} \right)^i\right) & \textrm{if i.i.d. (strategy $1$)} \\
        N_0 \left( \frac{1-p}{d} \right)^i \left( 1 - N_0\left( \frac{1-p}{d} \right)^i\right) & \textrm{if coupled (strategy $2$)}  
        \end{cases} & \textrm{if $i \geq 1$}.
    \end{cases}
\end{equation}
It is reassuring that the behaviours coincide when $N_0 = 1$. Note also that, with strategy $2$, we have the simple result 
\begin{equation}
    \mathbb{E}(N_i^2) = \mathbb{E}(N_i).
\end{equation}

In the special case $N_0 < d$, we also have that $\mathbb{E}(N_x N_y) = 0$ unless the walks $\omega_{ix}$ and $\omega_{iy}$ share only the first node $i$ and no further edges. It is possible to show this algebraically from the derived forms, or simply observe that it is only possible for the node labelled $i$ to accommodate more than one walker \textcolor{blue}{(rephrase)}. 

\subsection{Putting the pieces together}
The following table summarises the statistical behaviour of $N_{\omega_{ix}}N_{\omega_{iy}}$, supposing we start with $N_0$ walkers at node $i$. Let $\frac{1-p}{d} \coloneqq c$.

\begin{table}[H] \label{tab}
    \centering
    \tiny
\begin{tabular}{c| c c c }
\toprule
Pair class & \multicolumn{3}{c}{$\mathbb{E}(N_x N_y )$}  \\
 & Strategy 1 (i.i.d) & Strategy 2 (coupled) & Difference \\
\midrule
Same walk, $\omega_{ix} = \omega_{iy}$ & $N_0 c^{\omega_{ix}} + N_0(N_0 - 1) c^{2{\omega_{ix}}}$ & $N_0c^{\omega_{ix}}$ & $N_0(N_0-1)c^{2\omega_{ix}}$ \\ 
Subwalk, $\omega_{ix} \in \omega_{iy}$ & $N_0 c^{\omega_{iy}} + N_0(N_0 - 1) c^{\omega_{ix} + \omega_{iy}}$ &$N_0c^{\omega_{iy}}$ & $N_0(N_0-1)c^{\omega_{ix} + \omega_{iy}}$\\
Different walks, diverge at $i$ & $N_0(N_0-1)c^{\omega_{ix}+\omega_{iy}}$ & $\frac{d}{d-1} N_0(N_0-1)c^{\omega_{ix}+\omega_{iy}}$ & $-\frac{1}{d-1} N_0(N_0-1)c^{\omega_{ix}+\omega_{iy}}$\\
Different walks, diverge at $d \neq i$ & $N_0(N_0-1)c^{\omega_{ix}+\omega_{iy}}$ & $0$ & $N_0(N_0-1)c^{\omega_{ix}+\omega_{iy}}$ \\
\bottomrule
\end{tabular}
\end{table}
It is interesting and nontrivial to observe that the \emph{difference} in correlation terms adopts a simple form for all pairwise walk behaviours. Were it not for the negative sign in `different walks', our task would be done. Unfortunately this is not the case.

We need to think about the quantity
\begin{equation}
\begin{multlined}
    \mathbb{E}(\phi(i)^\top \phi(j)) = \frac{1}{N^2} \sum_x \sum_y \left( \sum_{\omega_{ix} \in \Omega_{ix}} \sum_{\omega_{iy} \in \Omega_{iy}} \frac{\widetilde{\omega}(\omega_{ix})}{p(\omega_{ix})} \frac{\widetilde{\omega}(\omega_{iy})}{p(\omega_{iy})} \mathbb{E} ( N(\omega_{ix}) N(\omega_{iy}) ) \right)
    \\ \cdot \left( \sum_{\omega_{jx} \in \Omega_{jx}} \sum_{\omega_{jy} \in \Omega_{jy}} \frac{\widetilde{\omega}(\omega_{jx})}{p(\omega_{jx})} \frac{\widetilde{\omega}(\omega_{jy})}{p(\omega_{jy})} \mathbb{E} ( N(\omega_{jx}) N(\omega_{jy}) ) \right)
\end{multlined}
\end{equation}
and show that it's reduced in the new scheme.

From quick numerical experiments, it does \emph{not} seem to be the case that the terms in curly parentheses are always reduced for all $(x,y)$. I think we might have to do a beastly spectral treatment like in the q-GRFs paper.

Going to have to get spectral and do sum over x and y. Roll sleeves up and do the integrals. 

\subsection{Doing some integrals -- a new hope?}
First consider the simpler problem of making the walks out of one of the nodes $j$ repelling, whilst leaving $i$ unchanged. Various terms appear \textcolor{blue}{[to do: enumerate]}, for example
\begin{equation}
\begin{multlined}
    \sum_{xy} \left( \sum_{k_1} \sum_{k_2} \frac{w\lambda_{k_1}}{1-w\lambda_{k_1}} \frac{w\lambda_{k_2}}{1-w\lambda_{k_2}}  \braket{i|k_1} \braket{k_1|x} \braket{i|k_2} \braket{k_2|y}  \right)
    \\ \cdot \left( \sum_z \textrm{A}_{jz} \sum_{n=0}^\infty \textrm{A}^n_{zx} w^n \sum_{m=0}^\infty \textrm{A}^m_{zy} w^m - \frac{w^2}{d}  \sum_{n=1}^\infty \textrm{A}^n_{jx} w^n \sum_{m=1}^\infty \textrm{A}^m_{jy} w^m\right)
\end{multlined}
\end{equation}
where the second bracketed term comes from the column labelled `difference'. It can be rewritten
\begin{equation}
\sum_{k_3} \sum_{k_4} \braket{k_3|x} \braket{k_4|y} 
    \frac{w}{1-w\lambda_{k_3}} \frac{w}{1-w\lambda_{k_4}} 
    \left[\sum_z \textrm{A}_{jz} \braket{z|k_3} \braket{z|k_4} - \frac{\lambda_{k_3} \lambda_{k_4}}{d} \braket{j|k_3} \braket{j|k_4} \right]. 
\end{equation}
The sums over $x$ and $y$ resolve the identity, so we are left with
\begin{equation}
    \sum_{k_1} \sum_{k_2} \frac{w^2 \lambda_{k_1}}{(1 - w\lambda_{k_1})^2} \frac{w^2 \lambda_{k_2}}{(1 - w\lambda_{k_2})^2} \braket{i|k_1} \braket{i|k_2}\left[\sum_z \textrm{A}_{jz} \braket{z|k_1} \braket{z|k_2} - \frac{\lambda_{k_1} \lambda_{k_2}}{d} \braket{j|k_1} \braket{j|k_2} \right] 
\end{equation}
The second term can be written
\begin{equation} 
\frac{1}{d}\left(\bra{i} \frac{w^2 \textrm{A}^2 }{(1 - w \textrm{A} )^2 } \ket{j}\right)^2
\end{equation}
whilst the first term can be written
\begin{equation}
    \sum_{j' \sim j} \left(\bra{i} \frac{w^2 \textrm{A} }{(1 - w \textrm{A} )^2 } \ket{j'}\right)^2.
\end{equation}
Where $j' \sim j$ denotes the set of nodes adjacent to $j$. Now we make the simple observation that 
 \begin{equation}
     \textrm{A}\ket{j} = \sum_{j'} \ket{j'}
 \end{equation}
whereupon we need to determine if
\begin{equation}
   \sum_{j' \sim j} \left(\bra{i} \frac{w^2 \textrm{A} }{(1 - w \textrm{A} )^2 } \ket{j'}\right)^2 \overset{?}{\geq} \frac{1}{d}\left( \sum_{j' \sim j} \bra{i} \frac{w^2 \textrm{A} }{(1 - w \textrm{A} )^2 } \ket{j'}\right)^2. 
\end{equation}
This is trivially true by Jensen's inequality. 

We also need to think about terms where the LHS $\sim N_0 c^{\omega_{ix}}$, from consideration of the same walk/subwalks. These terms always look like
\begin{equation}
\begin{multlined}
    \sum_{xy} \sum_{\omega_{ix} \in \Omega_{ix}} \sum_{\omega_{iy} \in \Omega_{iy}} \left( \frac{wd}{1-p}\right)^{\textrm{len}(\omega_{ix}) + \textrm{len}(\omega_{iy})} \left\{ \mathbb{I}(\textrm{same walk})\left( \frac{1-p}{d}\right)^{\textrm{len}(\omega_{ix})}  \right.
    \\ \left. + \mathbb{I}(i \to x \to y) \left(\frac{1-p}{d}\right)^{\textrm{len}(\omega_{iy})} + \mathbb{I}(i \to y \to x) \left(\frac{1-p}{d}\right)^{\textrm{len}(\omega_{ix})}\right \} 
    \\ \cdot \left \{ \sum_{k_3} \sum_{k_4} \braket{k_3|x} \braket{k_4|y} \frac{w}{1-w\lambda_{k_3}} \frac{w}{1-w\lambda_{k_4}} \left[\sum_{j'} \braket{j'|k_3} \braket{j'|k_4}  - \frac{\lambda_{k_3}\lambda_{k_4}}{d} \braket{j|k_3} \braket{j|k_4} \right] \right \}.
\end{multlined}
\end{equation}
After a bit of work, we get
\begin{equation}
\begin{multlined}
    \sum_x \sum_{\omega_{ix} \in \Omega_{ix}}\left( \frac{w^2 d}{1-p}\right)^{\textrm{len}(\omega_{ix})} \sum_{k_3 k_4} \frac{1 - w^2 \lambda_{k_3} \lambda_{k_4}}{(1-w\lambda_{k_3})(1-w\lambda_{k_4})}
    \\ \cdot \left \{ \braket{k_3|x} \braket{k_4|x} \frac{w}{1-w\lambda_{k_3}} \frac{w}{1-w\lambda_{k_4}} \left[\sum_{j'} \braket{j'|k_3} \braket{j'|k_4}  - \frac{\lambda_{k_3}\lambda_{k_4}}{d} \braket{j|k_3} \braket{j|k_4} \right] \right \}.
\end{multlined}
\end{equation}
The prefactor is positive for every node $x$, so it is sufficient to consider the sign of the sum over $k_3$ and $k_4$. 

\textcolor{blue}{TO CHECK: maybe we have to make another small $w$ argument :(. Can say nonrestrictive in practice. Do numerical experiments. Sad because thought would always be true. Also need to check behaviour for terms corresponding to walks diverging at $i$ -- final bootstrap term. Annoyingly seems a pain.}

Seems always helpful when swapping walker out of first node $i$ to repelling, but next less clear. Still work to do to get all consistent.

\textcolor{red}{UPDATE: large $N_0$ (and hence implicitly large $d$ since $N_0 < d_\textrm{max}$) works. Will write up full proof ASAP. Will check but suspect generalisation to non $d$-regular will be easy enough. Small $N_0$, including regime where $N_0<d_\textrm{max}$, likely to be tricky.}

==> references.tex <==
\begin{thebibliography}{44}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Alon et~al.(2007)Alon, Benjamini, Lubetzky, and Sodin]{alon2007non}
Noga Alon, Itai Benjamini, Eyal Lubetzky, and Sasha Sodin.
\newblock Non-backtracking random walks mix faster.
\newblock \emph{Communications in Contemporary Mathematics}, 9\penalty0
  (04):\penalty0 585--603, 2007.
\newblock URL \url{https://doi.org/10.1142/S021919970700255}.

\bibitem[Amico et~al.(2008)Amico, Fazio, Osterloh, and
  Vedral]{amico2008entanglement}
Luigi Amico, Rosario Fazio, Andreas Osterloh, and Vlatko Vedral.
\newblock Entanglement in many-body systems.
\newblock \emph{Reviews of modern physics}, 80\penalty0 (2):\penalty0 517,
  2008.
\newblock URL \url{https://doi.org/10.1103/RevModPhys.80.517}.

\bibitem[Amit et~al.(1983)Amit, Parisi, and Peliti]{amit1983asymptotic}
Daniel~J Amit, Giorgio Parisi, and Luca Peliti.
\newblock Asymptotic behavior of the" true" self-avoiding walk.
\newblock \emph{Physical Review B}, 27\penalty0 (3):\penalty0 1635, 1983.
\newblock URL \url{https://doi.org/10.1103/PhysRevB.27.1635}.

\bibitem[Avrachenkov et~al.(2007)Avrachenkov, Litvak, Nemirovsky, and
  Osipova]{avrachenkov2007monte}
Konstantin Avrachenkov, Nelly Litvak, Danil Nemirovsky, and Natalia Osipova.
\newblock Monte carlo methods in pagerank computation: When one iteration is
  sufficient.
\newblock \emph{SIAM Journal on Numerical Analysis}, 45\penalty0 (2):\penalty0
  890--904, 2007.
\newblock URL \url{https://dl.acm.org/doi/10.1137/050643799}.

\bibitem[Becchetti et~al.(2008)Becchetti, Boldi, Castillo, and
  Gionis]{becchetti2008efficient}
Luca Becchetti, Paolo Boldi, Carlos Castillo, and Aristides Gionis.
\newblock Efficient semi-streaming algorithms for local triangle counting in
  massive graphs.
\newblock In \emph{Proceedings of the 14th ACM SIGKDD international conference
  on Knowledge discovery and data mining}, pages 16--24, 2008.
\newblock URL \url{https://dl.acm.org/doi/10.1145/1401890.1401898}.

\bibitem[Borgwardt et~al.(2005)Borgwardt, Ong, Sch{\"o}nauer, Vishwanathan,
  Smola, and Kriegel]{borgwardt2005protein}
Karsten~M Borgwardt, Cheng~Soon Ong, Stefan Sch{\"o}nauer, SVN Vishwanathan,
  Alex~J Smola, and Hans-Peter Kriegel.
\newblock Protein function prediction via graph kernels.
\newblock \emph{Bioinformatics}, 21\penalty0 (suppl\_1):\penalty0 i47--i56,
  2005.
\newblock URL \url{https://doi.org/10.1093/bioinformatics/bti1007}.

\bibitem[Chen(2014)]{chen2014two}
Jun Chen.
\newblock {Two particles' repelling random walks on the complete graph}.
\newblock \emph{Electronic Journal of Probability}, 19\penalty0
  (none):\penalty0 1 -- 17, 2014.
\newblock \doi{10.1214/EJP.v19-2669}.
\newblock URL \url{https://doi.org/10.1214/EJP.v19-2669}.

\bibitem[Chen et~al.(2016)Chen, Li, Wang, and Lui]{chen2016general}
Xiaowei Chen, Yongkun Li, Pinghui Wang, and John Lui.
\newblock A general framework for estimating graphlet statistics via random
  walk.
\newblock \emph{arXiv preprint arXiv:1603.07504}, 2016.
\newblock URL \url{https://doi.org/10.48550/arXiv.1603.07504}.

\bibitem[Choromanski et~al.(2018)Choromanski, Rowland, Sindhwani, Turner, and
  Weller]{choromanski2018structured}
Krzysztof Choromanski, Mark Rowland, Vikas Sindhwani, Richard Turner, and
  Adrian Weller.
\newblock Structured evolution with compact architectures for scalable policy
  optimization.
\newblock In \emph{International Conference on Machine Learning}, pages
  970--978. PMLR, 2018.
\newblock URL \url{https://doi.org/10.48550/arXiv.1603.07504}.

\bibitem[Choromanski et~al.(2020)Choromanski, Likhosherstov, Dohan, Song, Gane,
  Sarlos, Hawkins, Davis, Mohiuddin, Kaiser, et~al.]{choromanski2020rethinking}
Krzysztof Choromanski, Valerii Likhosherstov, David Dohan, Xingyou Song,
  Andreea Gane, Tamas Sarlos, Peter Hawkins, Jared Davis, Afroz Mohiuddin,
  Lukasz Kaiser, et~al.
\newblock Rethinking attention with performers.
\newblock \emph{arXiv preprint arXiv:2009.14794}, 2020.
\newblock URL \url{https://doi.org/10.48550/arXiv.2009.14794}.

\bibitem[Choromanski et~al.(2017)Choromanski, Rowland, and
  Weller]{choromanski2017unreasonable}
Krzysztof~M Choromanski, Mark Rowland, and Adrian Weller.
\newblock The unreasonable effectiveness of structured random orthogonal
  embeddings.
\newblock \emph{Advances in neural information processing systems}, 30, 2017.
\newblock URL \url{https://doi.org/10.48550/arXiv.1703.00864}.

\bibitem[Choromanski(2023)]{choromanski2023taming}
Krzysztof~Marcin Choromanski.
\newblock Taming graph kernels with random features.
\newblock In \emph{International Conference on Machine Learning}, pages
  5964--5977. PMLR, 2023.
\newblock URL \url{https://doi.org/10.48550/arXiv.2305.00156}.

\bibitem[Chung and Yau(1999)]{chung}
Fan R.~K. Chung and Shing{-}Tung Yau.
\newblock Coverings, heat kernels and spanning trees.
\newblock \emph{Electron. J. Comb.}, 6, 1999.
\newblock \doi{10.37236/1444}.
\newblock URL \url{https://doi.org/10.37236/1444}.

\bibitem[Chung(1997)]{chung1997spectral}
Fan~RK Chung.
\newblock \emph{Spectral graph theory}, volume~92.
\newblock American Mathematical Soc., 1997.

\bibitem[Crane et~al.(2017)Crane, Weischedel, and Wardetzky]{crane2017heat}
Keenan Crane, Clarisse Weischedel, and Max Wardetzky.
\newblock The heat method for distance computation.
\newblock \emph{Communications of the ACM}, 60\penalty0 (11):\penalty0 90--99,
  2017.
\newblock URL \url{https://dl.acm.org/doi/10.1145/3131280}.

\bibitem[Dawson-Haggerty(2023)]{trimesh}
Michael Dawson-Haggerty.
\newblock Trimesh repository, 2023.
\newblock URL \url{https://github.com/mikedh/trimesh}.

\bibitem[Dhillon et~al.(2004)Dhillon, Guan, and Kulis]{dhillon2004kernel}
Inderjit~S Dhillon, Yuqiang Guan, and Brian Kulis.
\newblock Kernel k-means: spectral clustering and normalized cuts.
\newblock In \emph{Proceedings of the tenth ACM SIGKDD international conference
  on Knowledge discovery and data mining}, pages 551--556, 2004.
\newblock URL \url{https://dl.acm.org/doi/10.1145/1014052.1014118}.

\bibitem[Diaconis et~al.(2000)Diaconis, Holmes, and Neal]{diaconis2000analysis}
Persi Diaconis, Susan Holmes, and Radford~M Neal.
\newblock Analysis of a nonreversible markov chain sampler.
\newblock \emph{Annals of Applied Probability}, pages 726--752, 2000.
\newblock URL \url{https://doi.org/10.1214/aoap/1019487508}.

\bibitem[Dick et~al.(2013)Dick, Kuo, and Sloan]{dick2013high}
Josef Dick, Frances~Y Kuo, and Ian~H Sloan.
\newblock High-dimensional integration: the quasi-monte carlo way.
\newblock \emph{Acta Numerica}, 22:\penalty0 133--288, 2013.
\newblock URL \url{https://doi.org/10.1017/S0962492913000044}.

\bibitem[Doshi et~al.(2023)Doshi, Hu, and Eun]{doshi2023self}
Vishwaraj Doshi, Jie Hu, and Do~Young Eun.
\newblock Self-repellent random walks on general graphs--achieving minimal
  sampling variance via nonlinear markov chains.
\newblock \emph{arXiv preprint arXiv:2305.05097}, 2023.
\newblock URL \url{https://doi.org/10.48550/arXiv.2305.05097}.

\bibitem[Fogaras et~al.(2005)Fogaras, R{\'a}cz, Csalog{\'a}ny, and
  Sarl{\'o}s]{fogaras2005towards}
D{\'a}niel Fogaras, Bal{\'a}zs R{\'a}cz, K{\'a}roly Csalog{\'a}ny, and
  Tam{\'a}s Sarl{\'o}s.
\newblock Towards scaling fully personalized pagerank: Algorithms, lower
  bounds, and experiments.
\newblock \emph{Internet Mathematics}, 2\penalty0 (3):\penalty0 333--358, 2005.
\newblock URL \url{https://doi.org/10.1007/978-3-540-30216-2_9}.

\bibitem[Ivashkin(2023)]{community_graphs}
Vladimir Ivashkin.
\newblock Community graphs repository, 2023.
\newblock URL \url{https://github.com/vlivashkin/community-graphs}.

\bibitem[Kloster and Gleich(2014)]{kloster2014heat}
Kyle Kloster and David~F Gleich.
\newblock Heat kernel based community detection.
\newblock In \emph{Proceedings of the 20th ACM SIGKDD international conference
  on Knowledge discovery and data mining}, pages 1386--1395, 2014.
\newblock URL \url{https://doi.org/10.48550/arXiv.1403.3148}.

\bibitem[Lee et~al.(2012)Lee, Xu, and Eun]{lee2012beyond}
Chul-Ho Lee, Xin Xu, and Do~Young Eun.
\newblock Beyond random walk and metropolis-hastings samplers: why you should
  not backtrack for unbiased graph sampling.
\newblock \emph{ACM SIGMETRICS Performance evaluation review}, 40\penalty0
  (1):\penalty0 319--330, 2012.
\newblock URL \url{https://dl.acm.org/doi/10.1145/2318857.2254795}.

\bibitem[Milenkovi{\'c} and Pr{\v{z}}ulj(2008)]{milenkovic2008uncovering}
Tijana Milenkovi{\'c} and Nata{\v{s}}a Pr{\v{z}}ulj.
\newblock Uncovering biological network function via graphlet degree
  signatures.
\newblock \emph{Cancer informatics}, 6:\penalty0 CIN--S680, 2008.
\newblock URL \url{https://doi.org/10.48550/arXiv.0802.0556}.

\bibitem[Milo et~al.(2002)Milo, Shen-Orr, Itzkovitz, Kashtan, Chklovskii, and
  Alon]{milo2002network}
Ron Milo, Shai Shen-Orr, Shalev Itzkovitz, Nadav Kashtan, Dmitri Chklovskii,
  and Uri Alon.
\newblock Network motifs: simple building blocks of complex networks.
\newblock \emph{Science}, 298\penalty0 (5594):\penalty0 824--827, 2002.
\newblock URL \url{https://www.science.org/doi/10.1126/science.298.5594.824}.

\bibitem[Page et~al.(1998)Page, Brin, Motwani, and Winograd]{page1998pagerank}
Lawrence Page, Sergey Brin, Rajeev Motwani, and Terry Winograd.
\newblock The pagerank citation ranking: Bring order to the web.
\newblock Technical report, Technical report, stanford University, 1998.
\newblock URL
  \url{https://www.cis.upenn.edu/~mkearns/teaching/NetworkedLife/pagerank.pdf}.

\bibitem[Pemantle(2007)]{pemantle2007survey}
Robin Pemantle.
\newblock {A survey of random processes with reinforcement}.
\newblock \emph{Probability Surveys}, 4\penalty0 (none):\penalty0 1 -- 79,
  2007.
\newblock \doi{10.1214/07-PS094}.
\newblock URL \url{https://doi.org/10.1214/07-PS094}.

\bibitem[Pr{\v{z}}ulj(2007)]{prvzulj2007biological}
Nata{\v{s}}a Pr{\v{z}}ulj.
\newblock Biological network comparison using graphlet degree distribution.
\newblock \emph{Bioinformatics}, 23\penalty0 (2):\penalty0 e177--e183, 2007.
\newblock URL \url{https://doi.org/10.1093/bioinformatics/btl301}.

\bibitem[Rahimi and Recht(2007)]{rahimi2007random}
Ali Rahimi and Benjamin Recht.
\newblock Random features for large-scale kernel machines.
\newblock \emph{Advances in neural information processing systems}, 20, 2007.
\newblock URL \url{https://dl.acm.org/doi/10.5555/2981562.2981710}.

\bibitem[Reid et~al.(2023{\natexlab{a}})Reid, Choromanski, and
  Weller]{reid2023quasi}
Isaac Reid, Krzysztof Choromanski, and Adrian Weller.
\newblock Quasi-monte carlo graph random features.
\newblock \emph{arXiv preprint arXiv:2305.12470}, 2023{\natexlab{a}}.
\newblock URL \url{https://doi.org/10.48550/arXiv.2305.12470}.

\bibitem[Reid et~al.(2023{\natexlab{b}})Reid, Choromanski, Likhosherstov, and
  Weller]{reid2023simplex}
Isaac Reid, Krzysztof~Marcin Choromanski, Valerii Likhosherstov, and Adrian
  Weller.
\newblock Simplex random features.
\newblock In \emph{International Conference on Machine Learning}, pages
  28864--28888. PMLR, 2023{\natexlab{b}}.
\newblock URL \url{https://doi.org/10.48550/arXiv.2301.13856}.

\bibitem[Rosales et~al.(2022)Rosales, Prado, and Pires]{rosales2022vertex}
Rafael~A Rosales, Fernando~PA Prado, and Benito Pires.
\newblock Vertex reinforced random walks with exponential interaction on
  complete graphs.
\newblock \emph{Stochastic Processes and their Applications}, 148:\penalty0
  353--379, 2022.
\newblock URL \url{https://doi.org/10.1016/j.spa.2022.03.007}.

\bibitem[Rowland et~al.(2018)Rowland, Choromanski, Chalus, Pacchiano, Sarlos,
  Turner, and Weller]{rowland2018geometrically}
Mark Rowland, Krzysztof~M Choromanski, Fran{\c{c}}ois Chalus, Aldo Pacchiano,
  Tamas Sarlos, Richard~E Turner, and Adrian Weller.
\newblock Geometrically coupled monte carlo sampling.
\newblock \emph{Advances in Neural Information Processing Systems}, 31, 2018.
\newblock URL \url{https://dl.acm.org/doi/pdf/10.5555/3326943.3326962}.

\bibitem[Rowland et~al.(2019)Rowland, Hron, Tang, Choromanski, Sarlos, and
  Weller]{rowland2019orthogonal}
Mark Rowland, Jiri Hron, Yunhao Tang, Krzysztof Choromanski, Tamas Sarlos, and
  Adrian Weller.
\newblock Orthogonal estimation of wasserstein distances.
\newblock In \emph{The 22nd International Conference on Artificial Intelligence
  and Statistics}, pages 186--195. PMLR, 2019.
\newblock URL \url{https://doi.org/10.48550/arXiv.1903.03784}.

\bibitem[Shervashidze et~al.(2009)Shervashidze, Vishwanathan, Petri, Mehlhorn,
  and Borgwardt]{shervashidze2009efficient}
Nino Shervashidze, SVN Vishwanathan, Tobias Petri, Kurt Mehlhorn, and Karsten
  Borgwardt.
\newblock Efficient graphlet kernels for large graph comparison.
\newblock In \emph{Artificial intelligence and statistics}, pages 488--495.
  PMLR, 2009.
\newblock URL \url{https://api.semanticscholar.org/CorpusID:17557614}.

\bibitem[Smola and Kondor(2003)]{smola2003kernels}
Alexander~J Smola and Risi Kondor.
\newblock Kernels and regularization on graphs.
\newblock In \emph{Learning Theory and Kernel Machines: 16th Annual Conference
  on Learning Theory and 7th Kernel Workshop, COLT/Kernel 2003, Washington, DC,
  USA, August 24-27, 2003. Proceedings}, pages 144--158. Springer, 2003.
\newblock URL
  \url{https://people.cs.uchicago.edu/~risi/papers/SmolaKondor.pdf}.

\bibitem[Tarrès(2004)]{tarres2004vertex}
Pierre Tarrès.
\newblock Vertex-reinforced random walk on z eventually gets stuck on five
  points.
\newblock \emph{The Annals of Probability}, 32\penalty0 (3):\penalty0
  2650--2701, 2004.
\newblock ISSN 00911798.
\newblock URL \url{http://www.jstor.org/stable/3481644}.

\bibitem[T{\'o}th(1995)]{toth1995true}
B{\'a}lint T{\'o}th.
\newblock The" true" self-avoiding walk with bond repulsion on z: Limit
  theorems.
\newblock \emph{The Annals of Probability}, pages 1523--1556, 1995.
\newblock URL \url{https://doi.org/10.1214/aop/1176987793}.

\bibitem[Ugander et~al.(2013)Ugander, Backstrom, and
  Kleinberg]{ugander2013subgraph}
Johan Ugander, Lars Backstrom, and Jon Kleinberg.
\newblock Subgraph frequencies: Mapping the empirical and extremal geography of
  large graph collections.
\newblock In \emph{Proceedings of the 22nd international conference on World
  Wide Web}, pages 1307--1318, 2013.
\newblock URL \url{https://doi.org/10.48550/arXiv.1304.1548}.

\bibitem[Xia et~al.(2019)Xia, Liu, Nie, Fu, Wan, and Kong]{xia2019random}
Feng Xia, Jiaying Liu, Hansong Nie, Yonghao Fu, Liangtian Wan, and Xiangjie
  Kong.
\newblock Random walks: A review of algorithms and applications.
\newblock \emph{IEEE Transactions on Emerging Topics in Computational
  Intelligence}, 4\penalty0 (2):\penalty0 95--107, 2019.
\newblock URL \url{https://doi.org/10.1109/TETCI.2019.2952908}.

\bibitem[Yu et~al.(2016)Yu, Suresh, Choromanski, Holtmann-Rice, and
  Kumar]{yu2016orthogonal}
Felix Xinnan~X Yu, Ananda~Theertha Suresh, Krzysztof~M Choromanski, Daniel~N
  Holtmann-Rice, and Sanjiv Kumar.
\newblock Orthogonal random features.
\newblock \emph{Advances in neural information processing systems}, 29, 2016.
\newblock URL \url{https://doi.org/10.48550/arXiv.1610.09072}.

\bibitem[Zhou et~al.(2020)Zhou, Chen, and Xu]{zhou2020learning}
Yufan Zhou, Changyou Chen, and Jinhui Xu.
\newblock Learning manifold implicitly via explicit heat-kernel learning.
\newblock \emph{Advances in Neural Information Processing Systems},
  33:\penalty0 477--487, 2020.
\newblock URL \url{https://doi.org/10.48550/arXiv.2010.01761}.

\bibitem[Zhou et~al.(2015)Zhou, Zhang, and Das]{zhou2015leveraging}
Zhuojie Zhou, Nan Zhang, and Gautam Das.
\newblock Leveraging history for faster sampling of online social networks.
\newblock \emph{arXiv preprint arXiv:1505.00079}, 2015.
\newblock URL \url{https://doi.org/10.48550/arXiv.1505.00079}.

\end{thebibliography}

